A Survey of Data Quality Measurement and Monitoring Tools

High-quality data is key to interpretable and trustworthy data analytics and the basis for meaningful data-driven decisions. In practical scenarios, data quality is typically associated with data preprocessing, profiling, and cleansing for subsequent tasks like data integration or data analytics. However, from a scientific perspective, a lot of research has been published about the measurement (i.e., the detection) of data quality issues and different generally applicable data quality dimensions and metrics have been discussed. In this work, we close the gap between research into data quality measurement and practical implementations by investigating the functional scope of current data quality tools. With a systematic search, we identified 667 software tools dedicated to "data quality", from which we evaluated 13 tools with respect to three functionality areas: (1) data profiling, (2) data quality measurement in terms of metrics, and (3) continuous data quality monitoring. We selected the evaluated tools with regard to pre-defined exclusion criteria to ensure that they are domain-independent, provide the investigated functions, and are evaluable freely or as trial. This survey aims at a comprehensive overview on state-of-the-art data quality tools and reveals potential for their functional enhancement. Additionally, the results allow a critical discussion on concepts, which are widely accepted in research, but hardly implemented in any tool observed, for example, generally applicable data quality metrics.

==> chapters/7_acks.tex <==
\begin{acks}
The research reported in this paper has been supported by the Austrian Ministry for Transport, Innovation and Technology, the Federal Ministry for Digital and Economic Affairs, and the Province of Upper Austria in the frame of the COMET center SCCH. 

The authors would like to thank all contact persons who provided us with trial licences and support, in particular, Thomas Bodenm{\"u}ller-Dodek and Dagmar Hillmeister-M{\"u}ller from Informatica, David Zydron from Experian, Alexis Rolland from Ubisoft,  Marc Kliffen from Human Inference, Ingo Lenzen from InfoZoom, Loredana Locci from SAS, and Rudolf Plank from solvistas GmbH. Special thanks to Alexander Gindlhumer for his support with Apache Griffin. 
\end{acks}

